Integrating Sustainability Concerns into Agile Software Development Process

Software has the potential to be a key driver in fostering sustainability. Despite this potential, it is not clear if and how the software industry integrates consideration of sustainability into its common software development processes. This research starts by investigating the current state of sustainability consideration within the software engineering industry through a survey. The results highlight a lack of progress in practically integrating sustainability considerations into software development activities. To address this gap, a case study with an industry partner is conducted to demonstrate how sustainability concerns and effects can be integrated into agile software development. The findings of this case study demonstrate practical approaches to integrating sustainability into software development practices. Reflecting on the findings from the survey and the case study, we note some insights on scaling up the adoption of sustainability consideration into the daily practice of agile software development.

==> sections/threat-validity.tex <==
% \section{Threat to Validity}\label{sec:threat-validity}

% We have presented a preliminary result of ongoing research towards integrating sustainability considerations into agile software development. This section details the threat to validity:  %\cite{wohlin2012experimentation}. The identified threats to validity include:

% \textbf{Internal validity:} To mitigate the threat of internal validity, this study utilized a mixed-methods approach, incorporating both quantitative and qualitative data to triangulate findings and ensure robustness. First, a survey was conducted to find the current state of practices for sustainability in agile software development practice. Afterward, a case study was carried out in collaboration with an industry partner to explore avenues for integrating sustainability into agile software development processes and practices. 

% \textbf{External validity:} The primary focus of this study was on agile software development practices and the integration of sustainability principles. One limitation is that the survey and case study were limited to software development practitioners in Europe. However, concerted efforts were made to mitigate this limitation by offering a comprehensive roadmap that can be adapted to suit various software development approaches within different organizational contexts and domains.

% \textbf{Construct validity:} In order to ensure the validity and reliability of the results, existing frameworks, literature studies, and expert (software development practitioners and researchers) input were used to operationalize study concepts including software development methods, agile methodologies, and sustainability integration in software development.

% \textbf{Reliability:} This study applied member checking and triangulation of data sources for data collection and analysis to enhance the reliability of findings. Furthermore, transparent reporting and documentation of methods were provided to promote the repeatability of the research process.
